Robust Mean Teacher for Continual and Gradual Test-Time Adaptation

Since experiencing domain shifts during test-time is inevitable in practice, test-time adaption (TTA) continues to adapt the model after deployment. Recently, the area of continual and gradual test-time adaptation (TTA) emerged. In contrast to standard TTA, continual TTA considers not only a single domain shift, but a sequence of shifts. Gradual TTA further exploits the property that some shifts evolve gradually over time. Since in both settings long test sequences are present, error accumulation needs to be addressed for methods relying on self-training. In this work, we propose and show that in the setting of TTA, the symmetric cross-entropy is better suited as a consistency loss for mean teachers compared to the commonly used cross-entropy. This is justified by our analysis with respect to the (symmetric) cross-entropy's gradient properties. To pull the test feature space closer to the source domain, where the pre-trained model is well posed, contrastive learning is leveraged. Since applications differ in their requirements, we address several settings, including having source data available and the more challenging source-free setting. We demonstrate the effectiveness of our proposed method 'robust mean teacher' (RMT) on the continual and gradual corruption benchmarks CIFAR10C, CIFAR100C, and Imagenet-C. We further consider ImageNet-R and propose a new continual DomainNet-126 benchmark. State-of-the-art results are achieved on all benchmarks.

==> CVPR 23_ RMT (1)/figures/grad_surface.tex <==
\begin{figure*}[t]
  \centering
      \begin{tabular}{cc}
        \includegraphics[width=3.3in]{figures/cross-entropy.pdf} &
        \includegraphics[width=3.3in]{figures/symmetric-cross-entropy.pdf} \\
        \includegraphics[width=3.3in]{figures/grad-cross-entropy.pdf} &
        \includegraphics[width=3.3in]{figures/grad-symmetric-cross-entropy.pdf}
      \end{tabular}
  \caption{Loss (top) and gradient (bottom) surface illustrated for the binary case of the cross-entropy loss $\mathcal{L}_\mathrm{CE}$ and the symmetric cross-entropy $\mathcal{L}_\mathrm{SCE}$ in dependence of the confidences $p$ and $q$ of the student and teacher, respectively.}
  \label{fig:grad_surface}
\end{figure*}

==> CVPR 23_ RMT (1)/figures/loss_surface.tex <==
\begin{figure*}[t]
  \centering
      \begin{tabular}{cc}
        \includegraphics[width=3.3in]{figures/cross-entropy.pdf} &
        \includegraphics[width=3.3in]{figures/symmetric-cross-entropy.pdf}
      \end{tabular}
  \caption{Loss surface illustrated for the binary case of the cross-entropy loss $\mathcal{L}_\mathrm{CE}$ and the symmetric cross-entropy $\mathcal{L}_\mathrm{SCE}$ in dependence of the confidences $p$ and $q$ of the student and teacher, respectively.}
  \label{fig:loss_surface}
\end{figure*}

==> CVPR 23_ RMT (1)/figures/overview.tex <==
\begin{figure}[t]
\centering
\def\svgwidth{200pt}    
\input{figures/Setup.pdf_tex}  
\caption{\textbf{RMT framework:} Before the adaptation, the student and teacher networks are initialized with source pre-trained weights. Source prototypes are extracted for each class and a mean teacher warm-up is performed. During test-time, the current test batch $\bm{x}_t^\mathrm{T}$ and an augmented version $\Tilde{\bm{x}}_t^\mathrm{T}$ are encoded by the student. Test features, augmented test features, and the nearest source prototypes based on the cosine similarity are used for the contrastive loss $\mathcal{L}_\mathrm{CL}$. Self-training is performed by using two symmetric cross-entropy losses. If source data is available, we uniformly sample a batch $(\bm{x}_i^\mathrm{S}, \bm{y}_i^\mathrm{S})$ from the source data and compute the cross-entropy loss $\mathcal{L}_{\mathrm{CE}}^\mathrm{S}$. The student is updated by minimizing the previously mentioned losses. The teacher is updated via an exponential moving average of the student's parameters.}
\label{fig:framework}
\end{figure}

==> CVPR 23_ RMT (1)/tables/ablation_components.tex <==
\begin{table}[!t] % use \begin{table*} for two column style 
\renewcommand{\arraystretch}{1.2}
\centering
\caption{Classification error rate~(\%) for different configurations averaged over 3 runs.} \label{tab:ablation-components}
\scalebox{0.92}{
\tabcolsep3pt
\begin{tabular}{l| ccccc|c}\hline
Method  & \rotatebox[origin=c]{70}{CIFAR10C} & \rotatebox[origin=c]{70}{ CIFAR100C } & \rotatebox[origin=c]{70}{ImageNet-C} & \rotatebox[origin=c]{70}{ImageNet-R} & \rotatebox[origin=c]{70}{DomNet-126} & Mean \\
\hline
MT ($\mathcal{L}_\mathrm{CE}$)           & 18.8 & 32.1 & 65.9 & 59.6 & 41.9 & 43.7 \\
\hline
MT ($\mathcal{L}_\mathrm{SCE}$)         & 17.9 & 31.5 & 62.8 & 57.3 & 39.7 & 41.8 \\
 + warm-up    & 16.7 & 30.6 & 61.3 & 55.0 & 38.8 & 40.5 \\
\hline
 \textbf{A} $\mathcal{L}_{\mathrm{ST}}$ & 18.0 & 31.2 & 61.9 & 57.2 & 39.1 & 41.5\\
 \textbf{B} + ensemble                & 17.1 & 30.5 & 60.1 & 56.5 & 36.8 & 40.2 \\
 \textbf{C} + contrastive             & 16.7 & 30.1 & 59.9 & 55.6 & 35.0 & 39.5 \\
  %\textbf{D} + src. replay           & 14.6 & \textbf{27.6} & 58.7 & 56.2 & \textbf{33.8} & 38.2 \\
 \textbf{D} + warm-up                 & 14.5 & 29.0 & 59.8 & 55.7 & 34.7 & 38.7 \\
 \textbf{E} + src. replay             & \textbf{13.9} & \textbf{27.6} & \textbf{57.9} & \textbf{55.5} & \textbf{33.9} & \textbf{37.8} \\
\hline
\end{tabular}}
\end{table}


==> CVPR 23_ RMT (1)/tables/corruption-continual.tex <==
\begin{table*}[!h]
\renewcommand{\arraystretch}{1.2}
\centering
\caption{Classification error rate~(\%) for the CIFAR10-to-CIFAR10C, CIFAR100-to-CIFAR100C, and ImageNet-to-ImageNet-C online continual test-time adaptation task on the highest corruption severity level 5. For CIFAR10C the results are evaluated on WideResNet-28, for CIFAR100C on ResNeXt-29, and for Imagenet-C, ResNet-50 is used. We report the performance of our method averaged over 5 runs.} \label{tab:continual-corruptions}
\scalebox{0.93}{
\tabcolsep3pt
\begin{tabular}{l|l|c|c|ccccccccccccccc|c}\hline
& \multicolumn{3}{l|}{Time} & \multicolumn{15}{l|}{$t\xrightarrow{\hspace*{12.2cm}}$}& \\ \hline
& Method & \rotatebox[origin=c]{90}{Source-free} & \rotatebox[origin=c]{90}{Updates} & \rotatebox[origin=c]{70}{Gaussian} & \rotatebox[origin=c]{70}{shot} & \rotatebox[origin=c]{70}{impulse} & \rotatebox[origin=c]{70}{defocus} & \rotatebox[origin=c]{70}{glass} & \rotatebox[origin=c]{70}{motion} & \rotatebox[origin=c]{70}{zoom} & \rotatebox[origin=c]{70}{snow} & \rotatebox[origin=c]{70}{frost} & \rotatebox[origin=c]{70}{fog}  & \rotatebox[origin=c]{70}{brightness} & \rotatebox[origin=c]{70}{contrast} & \rotatebox[origin=c]{70}{elastic} & \rotatebox[origin=c]{70}{pixelate} & \rotatebox[origin=c]{70}{jpeg} & Mean \\
\hline
\multirow{9}{*}{\rotatebox[origin=c]{90}{CIFAR10C}}& Source only & \ding{51} & - & 72.3 & 65.7 & 72.9 & 46.9 & 54.3 & 34.8 & 42.0 & 25.1 & 41.3 & 26.0 & 9.3 & 46.7 & 26.6 & 58.5 & 30.3 & 43.5 \\
& BN--1     & \ding{51} & - & 28.1 & 26.1 & 36.3 & 12.8 & 35.3 & 14.2 & 12.1 & 17.3 & 17.4 & 15.3 & 8.4 & 12.6 & 23.8 & 19.7 & 27.3 & 20.4 \\
& TENT-cont.& \ding{51} & 1 & 24.8 & 20.6 & 28.6 &	14.4 & 31.1 & 16.5 & 14.1 & 19.1 & 18.6 & 18.6 & 12.2 & 20.3 & 25.7 & 20.8 & 24.9 & 20.7\\
& AdaContrast & \ding{51} & 1 & 29.1 & 22.5 & 30.0 & 14.0 & 32.7 & 14.1 & 12.0 & 16.6 & 14.9 & 14.4 & 8.1 & 10.0 & 21.9 & 17.7 & 20.0 & 18.5\\
& CoTTA     & \ding{51} & 1 & 24.3 & 21.3 & 26.6 & 11.6 & 27.6 & 12.2 & 10.3 & 14.8 & 14.1 & 12.4 & 7.5 & 10.6 & 18.3 & 13.4 & 17.3 & 16.2 \\
& GTTA-MIX & \ding{55} & 4 & 23.4 & 18.3 & 25.5 & \textbf{10.1} & 27.3 & 11.6 & 10.1 & 14.1 & 13.0 & 10.9 & 7.4 & 9.0 & 19.4 & 14.5 & 19.8 & 15.6 \\
& RMT (ours)& \ding{51} & 1 & 21.9 & 18.6 & 24.1 & 10.8 & 23.6 & 12.0 & 10.4 & 13.0 & 12.4 & 11.4 & 8.3 & 10.1 & 15.2 & 11.3 & 14.6 & 14.5$\pm$0.09 \\
& RMT (ours)& \ding{55} & 1 & 21.7 & 18.6 & 24.2 & 10.3 & 24.0 & 11.2 & 9.5 & 12.1 & 11.7 & 10.3 & \textbf{7.0} & 8.7 & 14.8 & 10.5 & 14.5 & 13.9$\pm$0.07 \\
& RMT (ours)& \ding{55} & 4 & \textbf{20.8} & \textbf{16.5} & \textbf{20.5} & 10.4 & \textbf{20.1} & \textbf{10.8} & \textbf{9.2} & \textbf{11.0} & \textbf{10.4} & \textbf{9.7} & 7.3 & \textbf{8.0} & \textbf{12.3} & \textbf{8.7} & \textbf{11.6} & \textbf{12.5}$\pm$0.07 \\
\hline
\multirow{9}{*}{\rotatebox[origin=c]{90}{CIFAR100C}}& Source only & \ding{51} & - & 73.0&	68.0&	39.4&	29.3&	54.1&	30.8&	28.8&	39.5&	45.8&	50.3&	29.5&	55.1&	37.2	&74.7&	41.2&	46.4\\
& BN--1     & \ding{51} & - & 42.1 & 40.7 & 42.7 & 27.6 & 41.9 & 29.7 & 27.9 & 34.9 & 35.0 & 41.5 & 26.5 & 30.3 & 35.7 & 32.9 & 41.2 & 35.4 \\
& TENT-cont.& \ding{51} & 1 & 37.2 & 35.8 & 41.7 & 37.9 & 51.2 & 48.3 & 48.5 & 58.4 & 63.7 & 71.1 & 70.4 & 82.3 & 88.0 & 88.5 & 90.4 & 60.9 \\
& AdaContrast & \ding{51} & 1 & 42.3 & 36.8 & 38.6 & 27.7 & 40.1 & 29.1 & 27.5 & 32.9 & 30.7 & 38.2 & 25.9 & 28.3 & 33.9 & 33.3 & 36.2 & 33.4 \\
& CoTTA     & \ding{51} & 1 & 40.1 & 37.7 & 39.7 & 26.9 & 38.0 & 27.9 & 26.4 & 32.8 & 31.8 & 40.3 & 24.7 & 26.9 & 32.5 & 28.3 & 33.5 & 32.5 \\
& GTTA-MIX & \ding{55} & 4 & 36.4 & \textbf{32.1} & 34.0 & \textbf{24.4} & 35.2 & 25.9 & 23.9 & 28.9 & 27.5 & 30.9 & 22.6 & \textbf{23.4} & 29.4 & 25.5
& 33.3 & 28.9 \\
& RMT (ours)& \ding{51} & 1 & 38.5 & 34.4 & 35.4 & 26.4 & 32.7 & 27.0 & 25.0 & 27.5 & 27.6 & 30.0 & 24.0 & 25.8 & 27.0 & 25.2 & 28.4 & 29.0$\pm$0.17 \\
& RMT (ours)& \ding{55} & 1 & 37.4 & 33.8 & 34.3 & 24.8 & 32.0 & 25.3 & \textbf{23.6} & 26.2 & 26.2 & 28.9 & \textbf{21.9} & 23.5 & 25.4 & \textbf{23.2} & 27.4 & 27.6$\pm$0.04 \\
& RMT (ours)& \ding{55} & 4 & \textbf{36.2} & 32.2 & \textbf{32.1} & 25.0 & \textbf{29.8} & \textbf{25.0} & \textbf{23.6} & \textbf{25.4} & \textbf{25.2} & \textbf{27.1} & 23.1 & \textbf{23.4} & \textbf{24.4} & 23.4 & \textbf{25.9} & \textbf{26.8}$\pm$0.08 \\
\hline
\multirow{9}{*}{\rotatebox[origin=c]{90}{ImageNet-C}} & Source only & \ding{51} & - & 97.8 & 97.1 & 98.2 & 81.7 & 89.8 & 85.2 & 78.0 & 83.5 & 77.1 & 75.9 & 41.3 & 94.5 & 82.5 & 79.3 & 68.6 & 82.0 \\
 & BN--1     & \ding{51} & - & 85.0 & 83.7 & 85.0 & 84.7 & 84.3 & 73.7 & 61.2 & 66.0 & 68.2 & 52.1 & 34.9 & 82.7 & 55.9 & 51.3 & 59.8 & 68.6 \\
 & TENT-cont.& \ding{51} & 1 & 81.6 & 74.6 & 72.7 & 77.6 & 73.8 & 65.5 & 55.3 & 61.6 & 63.0 & 51.7 & 38.2 & 72.1 & 50.8 & 47.4 & 53.3 & 62.6 \\
 & AdaContrast & \ding{51} & 1 & 82.9 & 80.9 & 78.4 & 81.4 & 78.7 & 72.9 & 64.0 & 63.5 & 64.5 & 53.5 & 38.4 & 66.7 & 54.6 & 49.4 & 53.0 & 65.5 \\
 & CoTTA     & \ding{51} & 1 & 84.7 & 82.1 & 80.6 & 81.3 & 79.0 & 68.6 & 57.5 & 60.3 & 60.5 & 48.3 & 36.6 & 66.1 & 47.2 & 41.2 & 46.0 & 62.7 \\
 & GTTA-MIX & \ding{55} & 4 & 75.2 & \textbf{67.4} & \textbf{64.6} & 73.3 & 72.5 & 61.8 & \textbf{52.7} & \textbf{53.0} & \textbf{54.9} & \textbf{42.6} & \textbf{33.8} & 63.9 & 48.9 & 44.4 & 47.0 & 57.1 \\
 & RMT (ours)& \ding{51} & 1 & 77.9 & 73.1 & 69.9 & 73.5 & 71.1 & 63.1 & 57.1 & 57.1 & 59.2 & 50.4 & 42.9 & 60.1 & 49.0 & 45.7 & 46.9 & 59.8$\pm$0.18\\
 & RMT (ours)& \ding{55} & 1 & 77.3 & 73.2 & 71.1 & 73.1 & 71.2 & 61.2 & 53.7 & 54.3 & 58.0 & 46.1 & 38.2 & 58.5 & \textbf{45.4} & \textbf{42.3} & \textbf{44.5} & 57.9$\pm$0.26\\
 & RMT (ours)& \ding{55} & 4 & \textbf{74.8} & 68.6 & 65.2 & \textbf{68.2} & \textbf{66.2} & \textbf{59.0} & 53.4 & 53.7 & 56.9 & 47.5 & 41.2 & \textbf{54.1} & 46.0 & 44.6 & 45.9 & \textbf{56.4}$\pm$0.25\\
\hline
\end{tabular}}
\end{table*}

==> CVPR 23_ RMT (1)/tables/corruption-gradual.tex <==
\begin{table*}[!h]
\renewcommand{\arraystretch}{1.1}
\centering
\caption{Classification error rate~(\%) for the gradual CIFAR10-to-CIFAR10C, CIFAR100-to-CIFAR100C, and ImageNet-to-ImageNet-C benchmark averaged over all 15 corruptions. We separately report the performance averaged over all severity levels (@ level 1--5) and averaged only over the highest severity level 5 (@ level 5). The number in brackets denotes the difference to the continual benchmark.}
\label{tab:gradual-corruptions}
\scalebox{0.93}{
\tabcolsep3pt
\begin{tabular}{l|l|cccccccccc}\hline
& & Source & BN--1 & TENT-cont. & AdaCont. & CoTTA & GTTA-MIX & RMT & RMT  & RMT \\ \hline
& Source-free & \ding{51} & \ding{51}  & \ding{51} & \ding{51} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{55} \\ 
& Updates & - & - & 1 & 1 & 1 & 4 & 1 & 1  & 4 \\ \hline
\multirow{2}{*}{CIFAR10C} & @level 1--5  & 24.7 & 13.7 & 20.4 & 12.1 & 10.9 & 11.8 & 9.3 & \textbf{8.1} & 8.6\\
& @level 5 & 43.5 & 20.4 & 25.1 \small{(+4.4)} & 15.8 \small{(-2.7)} & 14.2 \small{(-2.0)} & 13.0 \small{(-2.6)} & 10.4 \small{(-4.1)} & 9.4 \small{(-4.5)} & \textbf{9.0} \small{(-3.5)} \\ 
\hline
\multirow{2}{*}{CIFAR100C} & @level 1--5 & 33.6 & 29.9 & 74.8 & 33.0 & 26.3 & 24.7  & 26.4 & \textbf{23.6} & 24.2 \\
& @level 5 & 46.4 & 35.4 & 75.9 \small{(+15.0)} & 35.9 \small{(+2.5)} & 28.3 \small{(-4.2)} & 26.1 \small{(-2.8)} & 26.9 \small{(-2.1)} & \textbf{24.3} \small{(-3.2)} & 24.5 \small{(-2.3)} \\ \hline
\multirow{2}{*}{Imagenet-C} & @level 1--5  & 58.4 & 48.3 & 46.4 & 66.3 & 38.8 & 37.7 & 39.3 & 37.8 & \textbf{36.8} \\
& @level 5 & 82.0 & 68.6 & 58.9 \small{(-3.7)} & 72.6 \small{(+7.1)} & 43.1 \small{(-19.6)} & 47.7 \small{(-9.4)} & 41.5 \small{(-18.3)} & 40.2 \small{(-17.7)} & \textbf{37.5} \small{(-18.9)} \\ \hline
\end{tabular}}
\end{table*}


==> CVPR 23_ RMT (1)/tables/inr_and_domnet.tex <==
\begin{table}[t] % use \begin{table*} for two column style
\renewcommand{\arraystretch}{1.2}
\centering
\caption{Classification error rate~(\%) for ImageNet-R and DomainNet-126 in the online continual TTA setting. We report the performance of our method averaged over 5 runs.} 
\label{tab:imagenetr_and_domainnet}
\scalebox{0.92}{
\tabcolsep3pt
\begin{tabular}{l|c|c|c||cccc|c}
\hline
\multicolumn{4}{c||}{} & \multicolumn{5}{c}{DomainNet-126} \\
\hline
Method  & \rotatebox[origin=c]{90}{ Source-free } & \rotatebox[origin=c]{90}{ Updates } & \rotatebox[origin=c]{70}{ImageNet-R} &\rotatebox[origin=c]{70}{real $\rightarrow$} & \rotatebox[origin=c]{70}{clipart $\rightarrow$} & \rotatebox[origin=c]{70}{painting $\rightarrow$} & \rotatebox[origin=c]{70}{sketch $\rightarrow$} & Mean \\
\hline
 Source only  & \ding{51} & - & 63.8 & 45.3 & 49.3 & 41.7 & 44.8 & 45.3 \\
 BN--1        & \ding{51} & - & 60.4 & 45.1 & 45.2 & 39.5 & 37.8 & 41.9 \\
 TENT cont.   & \ding{51} & 1 & 57.6 & 42.4 & 44.2 & 37.2 & 37.5 & 40.3 \\
 CoTTA        & \ding{51} & 1 & 57.4 & 43.4 & 43.0 & 36.4 & 36.3 & 39.8 \\
 AdaContrast  & \ding{51} & 1 & 59.1 & 37.8 & 37.6 & 32.3 & 31.9 & 34.9 \\
 GTTA-MIX     & \ding{55} & 4 & 56.6 & 38.7 & 42.4 & 33.6 & 34.2 & 37.2 \\
 RMT (ours)   & \ding{51} & 1 & 55.7 & 37.0 & 37.9 & 31.7 & 32.1 & 34.7 \\
 RMT (ours)   & \ding{55} & 1 & 55.5 & 36.8 & 37.1 & 30.6 & 31.1 & 33.9 \\
 RMT (ours)   & \ding{55} & 4 & \textbf{53.5} & \textbf{35.1} & \textbf{36.4} & \textbf{29.9} & \textbf{29.9} & \textbf{32.8}  \\
\hline
\end{tabular}}
\end{table}


==> CVPR 23_ RMT (1)/tables/sliding_window.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{1.2}
\centering
\caption{Classification error rate~(\%) for single-sample TTA.} \label{tab:sliding_window}
\scalebox{0.93}{
\tabcolsep3pt
\begin{tabular}{l|c|ccccc|c}\hline
Method & \rotatebox[origin=c]{90}{ Window size } & \rotatebox[origin=c]{70}{CIFAR10C} & \rotatebox[origin=c]{70}{CIFAR100C} & \rotatebox[origin=c]{70}{ImageNet-C} & \rotatebox[origin=c]{70}{ImageNet-R} & \rotatebox[origin=c]{70}{DomNet-126} & Mean  \\
\hline
Source only & -  & 43.5 & 46.4 & 82.0 & 63.8 & 45.3 & 56.2 \\
\hline
BN--1       & 8  & 26.3 & 43.8 & 74.6 & 64.7 & 49.7 & 51.8 \\
BN--1       & 16 & 23.2 & 39.5 & 71.0 & 62.2 & 45.4 & 48.3 \\
BN--1       & 32 & 21.9 & 37.4 & 69.3 & 60.7 & 43.4 & 46.5 \\
\hline
RMT (ours)  & 8  & 16.7 & 33.6 & 72.0 & 59.7 & 43.7 & 45.1 \\
RMT (ours)  & 16 & 15.2 & 30.8 & 63.9 & 57.8 & 36.8 & 40.9 \\
RMT (ours)  & 32 & 14.3 & 28.1 & 59.9 & 56.1 & 35.3 & 38.7 \\
\hline
\end{tabular}}
\end{table}

